Systematic uncertainties on DESI Tully-Fisher distances constrained with Integral Field Spectroscopy

The Tully--Fisher (TF) relation is an empirical tool for estimating distances to spiral galaxies. The Dark Energy Spectroscopic Instrument (DESI) Peculiar Velocity (PV) Survey uses \texttt{`tractor'} photometric position angles to place fibers along the galaxy's semi-major axis and infer maximum rotational velocities for $\approx$ 53,000 spirals. Systematic errors arise if the photometric PA differs from the kinematic PA from velocity fields. We quantify systematic uncertainties in DESI-TF distance estimates from photometric PAs and assess the impact of photometric--kinematic PA misalignments. We analyze 215 nearby galaxies from the PISCO and AMUSING surveys, estimating maximum rotational velocities at $0.4\,R_{26}$ for consistency with DESI-PV. Kinematic parameters are derived using \texttt{`PaFit'} from \texttt{`Cappellari Software'}. Global photometric parameters rely on Siena Galaxy Atlas SGA-2020 \texttt{`tractor'} data, with \texttt{`HostPhot'} as an alternative approach. Approximately $28\%$ of our sample exhibit photometric--kinematic PA misalignments $>10^\circ$. The median bias in distance is $\approx +1.98\,\mathrm{Mpc}$ with a skewed residual distribution of outliers. The overall distance standard deviation is $19.35\,\mathrm{Mpc}$, with misaligned galaxies showing twice the dispersion of aligned ones. The Mean Percentage Error is $2.8\% \pm 1.96$ (SE). High galaxy-to-galaxy scatter appears in DESI-TF distances, particularly for misaligned systems. Because DESI-TF targets lack kinematic PA measurements, we recommend a global fractional uncertainty of $\approx 3.5\%$. When kinematic information is available, aligned galaxies with offsets $<10^\circ$ are consistent with $\approx 1\%$ uncertainty, while strongly misaligned or incomplete systems warrant an upper threshold of $\approx 10\%$.

==> authorlist <==

\author{
Utsav Siwakoti\inst{1,2,3}%
\thanks{The associated data and code are available on Zenodo via DOI: \href{https://doi.org/10.5281/zenodo.17925385}{10.5281/zenodo.17925385}}%
\orcid{0000-0003-3633-0098},
Llu\'is Galbany\inst{1,4}\orcid{0000-0002-1296-6887}\thanks{\email{lgalbany@ice.csic.es}},
Kelly A.~Douglass\inst{5}\orcid{0000-0002-9540-546X}\thanks{\email{kjdouglass@u.rochester.edu}},
A.~de~la~Macorra\inst{6}\orcid{0000-0002-1769-1640}\thanks{\email{macorra@fisica.unam.mx}},
A.~Kremin\inst{7}\orcid{0000-0001-6356-7424}\thanks{\email{akremin@lbl.gov}},
B.~A.~Weaver\inst{8}\thanks{\email{benjamin.weaver@noirlab.edu}},
C.~Hahn\inst{9}\orcid{0000-0003-1197-0902}\thanks{\email{changhoon.hahn@utexas.edu}},
D.~Bianchi\inst{10,11}\orcid{0000-0001-9712-0006}\thanks{\email{davide.bianchi1@unimi.it}},
D.~Brooks\inst{12}\thanks{\email{david.brooks@ucl.ac.uk}},
D.~Sprayberry\inst{8}\thanks{\email{david.sprayberry@noirlab.edu}},
E.~Gazta\~naga\inst{1,4,13}\orcid{0000-0001-9632-0815}\thanks{\email{gaztanaga@gmail.com}},
E.~S\'anchez\inst{14}\orcid{0000-0002-9646-8198}\thanks{\email{eusebio.sanchez@ciemat.es}},
F.~Prada\inst{15}\orcid{0000-0001-7145-8674}\thanks{\email{fprada@iaa.es}},
G.~Gutierrez\inst{16}\thanks{\email{gaston@fnal.gov}},
G.~Rossi\inst{17}\thanks{\email{graziano@sejong.ac.kr}},
G.~Tarl\'e\inst{18}\orcid{0000-0003-1704-0781}\thanks{\email{gtarle@umich.edu}},
H.~Zou\inst{19}\orcid{0000-0002-6684-3997}\thanks{\email{zouhu@nao.cas.cn}},
I.~P\'erez-R\`afols\inst{20}\orcid{0000-0001-6979-0125}\thanks{\email{ignasi.perez.rafols@upc.edu}},
J.~Aguilar\inst{7}\thanks{\email{jaguilar@lbl.gov}},
J.~E.~Forero-Romero\inst{21,22}\orcid{0000-0002-2890-3725}\thanks{\email{je.forero@uniandes.edu.co}},
J.~Moustakas\inst{23}\orcid{0000-0002-2733-4559}\thanks{\email{jmoustakas@siena.edu}},
J.~Silber\inst{7}\orcid{0000-0002-3461-0320}\thanks{\email{jhsilber@lbl.gov}},
L.~Le~Guillou\inst{24}\orcid{0000-0001-7178-8868}\thanks{\email{llg@lpnhe.in2p3.fr}},
M.~Landriau\inst{7}\orcid{0000-0003-1838-8528}\thanks{\email{mlandriau@lbl.gov}},
M.~Manera\inst{25,26}\orcid{0000-0003-4962-8934}\thanks{\email{mmanera@ifae.es}},
P.~Doel\inst{12}\thanks{\email{apd@star.ucl.ac.uk}},
R.~Joyce\inst{8}\orcid{0000-0003-0201-5241}\thanks{\email{richard.joyce@noirlab.edu}},
R.~Miquel\inst{26,27}\thanks{\email{rmiquel@ifae.es}},
R.~Sharples\inst{28,29}\orcid{0000-0003-3449-8583}\thanks{\email{r.m.sharples@durham.ac.uk}},
S.~Ahlen\inst{30}\orcid{0000-0001-6098-7247}\thanks{\email{ahlen@bu.edu}},
S.~Ferraro\inst{7,31}\orcid{0000-0003-4992-7854}\thanks{\email{sferraro@lbl.gov}},
S.~Gontcho~A~Gontcho\inst{32}\orcid{0000-0003-3142-233X}\thanks{\email{satya@virginia.edu}},
S.~Nadathur\inst{13}\orcid{0000-0001-9070-3102}\thanks{\email{seshadri.nadathur@port.ac.uk}},
T.~Claybaugh\inst{7}\thanks{\email{tmclaybaugh@lbl.gov}},
W.~J.~Percival\inst{33,34,35}\orcid{0000-0002-0644-5727}\thanks{\email{will.percival@uwaterloo.ca}}
}

\institute{
Institute of Space Sciences (ICE,CSIC),Campus UAB,Carrer de Can Magrans s/n,E-08193 Bellaterra (Barcelona),Spain
\and Department of Physics,Kathmandu University,Dhulikhel 45200,Nepal
\and Department of Physics \& Astronomy,University of Kansas,1251 Wescoe Hall Drive,Lawrence,KS 66045,USA
\and Institut d'Estudis Espacials de Catalunya (IEEC),c/Esteve Terradas 1,Edifici RDIT,Campus PMT-UPC,08860 Castelldefels,Spain
\and Department of Physics \& Astronomy,University of Rochester,500 Joseph C.~Wilson Blvd.,Rochester,NY 14627,USA
\and Instituto de F\'isica,Universidad Nacional Aut\'onoma de M\'exico,Circuito de la Investigaci\'on Cient\'ifica,Ciudad Universitaria,Cd.~de~M\'exico C.P.~04510,M\'exico
\and Lawrence Berkeley National Laboratory,1 Cyclotron Road,Berkeley,CA 94720,USA
\and NSF NOIRLab,950 N.~Cherry Ave.,Tucson,AZ 85719,USA
\and Department of Astronomy,The University of Texas at Austin,Austin,TX 78712,USA
\and Dipartimento di Fisica ``Aldo Pontremoli'',Universit\`a degli Studi di Milano,Via Celoria 16,I-20133 Milano,Italy
\and INAF--Osservatorio Astronomico di Brera,Via Brera 28,20122 Milano,Italy
\and Department of Physics \& Astronomy,University College London,Gower Street,London WC1E 6BT,UK
\and Institute of Cosmology and Gravitation,University of Portsmouth,Dennis Sciama Building,Portsmouth PO1 3FX,UK
\and CIEMAT,Avenida Complutense 40,E-28040 Madrid,Spain
\and Instituto de Astrof\'isica de Andaluc\'ia (CSIC),Glorieta de la Astronom\'ia s/n,E-18008 Granada,Spain
\and Fermi National Accelerator Laboratory,PO Box 500,Batavia,IL 60510,USA
\and Department of Physics and Astronomy,Sejong University,209 Neungdong-ro,Gwangjin-gu,Seoul 05006,Republic of Korea
\and University of Michigan,500 S.~State Street,Ann Arbor,MI 48109,USA
\and National Astronomical Observatories,Chinese Academy of Sciences,A20 Datun Road,Chaoyang District,Beijing 100101,P.R.~China
\and Departament de F\'isica,EEBE,Universitat Polit\`ecnica de Catalunya,c/Eduard Maristany 10,08930 Barcelona,Spain
\and Departamento de F\'isica,Universidad de los Andes,Cra.~1 No.~18A--10,Edificio IP,CP 111711,Bogot\'a,Colombia
\and Observatorio Astron\'omico,Universidad de los Andes,Cra.~1 No.~18A--10,Edificio H,CP 111711,Bogot\'a,Colombia
\and Department of Physics and Astronomy,Siena University,515 Loudon Road,Loudonville,NY 12211,USA
\and Sorbonne Universit\'e,CNRS/IN2P3,Laboratoire de Physique Nucl\'eaire et de Hautes \'Energies (LPNHE),FR-75005 Paris,France
\and Departament de F\'isica,Serra H\'unter,Universitat Aut\`onoma de Barcelona,08193 Bellaterra (Barcelona),Spain
\and Institut de F\'isica d'Altes Energies (IFAE),The Barcelona Institute of Science and Technology,Edifici CN,Campus UAB,08193 Bellaterra,Spain
\and Instituci\'o Catalana de Recerca i Estudis Avan\c{c}ats (ICREA),Passeig de Llu\'is Companys 23,08010 Barcelona,Spain
\and Centre for Advanced Instrumentation,Department of Physics,Durham University,South Road,Durham DH1 3LE,UK
\and Institute for Computational Cosmology,Department of Physics,Durham University,South Road,Durham DH1 3LE,UK
\and Department of Physics,Boston University,590 Commonwealth Avenue,Boston,MA 02215,USA
\and University of California,Berkeley,110 Sproul Hall \#5800,Berkeley,CA 94720,USA
\and Department of Astronomy,University of Virginia,Charlottesville,VA 22904,USA
\and Department of Physics and Astronomy,University of Waterloo,200 University Ave.~W,Waterloo,ON N2L 3G1,Canada
\and Perimeter Institute for Theoretical Physics,31 Caroline St.~N,Waterloo,ON N2L 2Y5,Canada
\and Waterloo Centre for Astrophysics,University of Waterloo,200 University Ave.~W,Waterloo,ON N2L 3G1,Canada
}
